Detection Recovery in Online Multi-Object Tracking with Sparse Graph Tracker

In existing joint detection and tracking methods, pairwise relational features are used to match previous tracklets to current detections. However, the features may not be discriminative enough for a tracker to identify a target from a large number of detections. Selecting only high-scored detections for tracking may lead to missed detections whose confidence score is low. Consequently, in the online setting, this results in disconnections of tracklets which cannot be recovered. In this regard, we present Sparse Graph Tracker (SGT), a novel online graph tracker using higher-order relational features which are more discriminative by aggregating the features of neighboring detections and their relations. SGT converts video data into a graph where detections, their connections, and the relational features of two connected nodes are represented by nodes, edges, and edge features, respectively. The strong edge features allow SGT to track targets with tracking candidates selected by top-K scored detections with large K. As a result, even low-scored detections can be tracked, and the missed detections are also recovered. The robustness of K value is shown through the extensive experiments. In the MOT16/17/20 and HiEve Challenge, SGT outperforms the state-of-the-art trackers with real-time inference speed. Especially, a large improvement in MOTA is shown in the MOT20 and HiEve Challenge. Code is available at https://github.com/HYUNJS/SGT.

==> tables/HiEve_rebuttal.tex <==
% \begin{table}[t!]
% \centering
% \caption{
% Evaluation results of ours and recent online JDT models on the HiEve benchmark (private detection). For each metric, the best is bolded and the second best is underlined. \textbf{\dag}~indicates no extra training dataset.
% }
% \label{table:hieve_result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}l|ccccccc@{}}
%     \toprule
%     Method & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%     \midrule
%         DeepSORT \textbf{\dag} & 27.1 & 28.5 & 8.4 & 41.4 & 5894 & 42668 & 3122 \\
%         JDE \textbf{\dag} & 33.1 & 36.0 & 15.1 & \textbf{24.1} & 6318 & 43577 & 3747 \\
%         FairMOT \textbf{\dag} & 35.0 & 46.7 & 16.3 & 44.2 & 6523 & 37750 & \textbf{995} \\
%         CenterTrack  \textbf{\dag} & 40.9 & 45.1 & 10.8 & 32.2 & \underline{3208} & 36414 & 1568 \\
%         NewTracker & 46.4 & 43.2 & \textbf{26.3} & 30.8 & 4667 & \textbf{30489} & 2133 \\
%         \textbf{SGT (Ours)} \textbf{\dag} & \underline{47.2} & \textbf{53.7} & \underline{24.0} & \underline{28.8} & 4699 & \underline{30727} & \underline{1361} \\
%         CSTrack & \textbf{48.6} & \underline{51.4} & 20.4 & 33.5 & \textbf{2366} & 31933 & 1475 \\
%     \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[t!]
\centering
\caption{
Comparison of ours and online JDT models on the HiEve benchmark (private detection). \textbf{\dag}~indicates no extra datasets.
}
\label{table:hieve_rebuttal}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    Method & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
    \midrule
        % DeepSORT \textbf{\dag} & 27.1 & 28.5 & 8.4 & 41.4 & 5894 & 42668 & 3122 \\
        % JDE \textbf{\dag} & 33.1 & 36.0 & 15.1 & 24.1 & 6318 & 43577 & 3747 \\
        FairMOT \textbf{\dag} & 35.0 & 46.7 & 16.3 & 44.2 & 6523 & 37750 & 995 \\
        CenterTrack  \textbf{\dag} & 40.9 & 45.1 & 10.8 & 32.2 & 3208 & 36414 & 1568 \\
        NewTracker & 46.4 & 43.2 & 26.3 & 30.8 & 4667 & 30489 & 2133 \\
        \textbf{SGT (Ours)} \textbf{\dag} & 47.2 & 53.7 & 24.0 & 28.8 & 4699 & 30727 & 1361 \\
        CSTrack & 48.6 & 51.4 & 20.4 & 33.5 & 2366 & 31933 & 1475 \\
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/design_edge_feat.tex <==
\begin{table}[t!]
\centering
\caption{Effect of choosing different relational features for initializing edge feature.}
\label{table:design_edge_feat}
\resizebox{\linewidth}{!}{
    \begin{tabular}{ @{} c | c c c c c c @{}}
        \toprule
        Combination of features & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$  \\
        \midrule
        x, y, w, h, IoU, Sim & \textbf{71.3} & \textbf{73.8} & \textbf{46.6} & 2190 & \textbf{12742} & \textbf{588} \\
        x, y, w, h, IoU & 69.9 & 71.5 & 44.8 & 1953 & 13508 & 821 \\
        x, y, w, h & 70.4 & 70.6 & 45.7 & 2113 & 13205 & 704 \\
        x, y & 69.6 & 70.3 & 43.1 & \textbf{1691} & 13899 & 837 \\
        IoU, Sim & 69.6 & 72.1 & 43.7 & 2066 & 13272 & 640 \\
        \bottomrule
    \end{tabular}
}
\end{table}

==> tables/mot_result_rebuttal.tex <==

% \begin{table}[t!]
% % \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \caption{
% Evaluation results of ours and recent online JDT models on the MOT17/20 benchmarks (private detection). \textbf{\dag}~indicates no extra training dataset.
% }
% \label{table:sgt_mot_rebuttal}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}l|ccccccc@{}}
%     \toprule
%     Method & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%     \midrule
%     \midrule
%     \multicolumn{8}{c}{MOT17 \cite{mot16}} \\
%     \midrule
%         CTracker \textbf{\dag} & 66.6 & 57.4 & 32.2 & 24.2 & 22284 & 160491 & 5529 \\
%         CenterTrack & 67.8 & 64.7 & 34.6 & 24.6 & \textbf{18489} & 160332 & \underline{3039} \\
%         QDTrack \dag & 68.7 & 66.3 & 40.6 & 21.9 & 26598 & 146643 & 3378 \\
%         TraDes & 69.1 & 63.9 & 36.4 & 21.5 & \underline{20892} & 150060 & 3555 \\
%         FairMOT \dag & 69.8 & 69.9 & - & - & - & - & 3996 \\
%         SOTMOT & 71.0 & 71.9 & 42.7 & 15.3 & 39537 & 118983 & 5184 \\
%         % FairMOT \cite{fairmot} & 71.9 & 72.3 & - & - & 18801 & 136821 & 2655 \\ % tuning threshold values by us
%         GSDT & 73.2 & 66.5 & 41.7 & 17.5 & 26397 & 120666 & 3891 \\
%         \textbf{SGT (Ours)} \dag & 73.2 & 70.2 & 42.0 & 17.7 & 25332 & 121155 & 4809 \\
%     \midrule
%     \multicolumn{8}{c}{MOT20 \cite{mot20}} \\
%     \midrule 
%         % FairMOT & 62.3 & 66.7 & 60.7 & 9.8 & 78431 & 111488 & 5073 \\ % tuning threshold values by us
%         % TransTrack \cite{transtrack} & \\
%         FairMOT & 61.8 & 67.3 & 68.8 & 7.6 & 103440 & 88901 & 5243\\
%         TransTrack & 64.5 & 59.2 & 49.1 & 13.6 & 28566 & 151377 & 3565 \\
%         \textbf{SGT (Ours)} \dag & 64.5 & 62.7 & 62.7 & 10.2 & 67352 & 111201 & 4909 \\
%     \bottomrule
% \end{tabular}
% }
% \end{table}

% \begin{table}[t!]
% \caption{
% Evaluation results of ours and recent online JDT models on the MOT16/17/20 benchmarks (private detection). The values not provided are filled by ``-''. \textbf{\dag}~indicates no extra training dataset.
% }
% \label{table:sgt_mot_rebuttal}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}l|ccccccc@{}}
%     \toprule
%     Method & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%     \midrule
%     \midrule
%     \multicolumn{8}{c}{MOT16 \cite{mot16}} \\
%     \midrule
%         QDTrack \cite{quasi-dense} \textbf{\dag} & 69.8 & 67.1 & 41.6 & 19.8 & 9861 & 44050 & 1097 \\
%         TraDes \cite{trades} & 70.1 & 64.7 & 37.3 & 20.0 & 8091 & 45210 & 1144 \\
%         CSTrack \cite{cstrack} \textbf{\dag} & 71.3 & 68.6 & - & - & - & - & 1356 \\
%         \textbf{SGT (Ours)} \textbf{\dag} & 74.1 & 71.0 & 43.6 & 15.8 & 9784 & 35946 & 1528 \\
%         GSDT \cite{gsdt} & 74.5 & 68.1 & 41.2 & 17.3 & 8913 & 36428 & 1229 \\
%         FairMOT \cite{fairmot} & 74.9 & 72.8 & 44.7 & 15.9 & - & - & 1074 \\
%     \midrule
%     \multicolumn{8}{c}{MOT17 \cite{mot16}} \\
%     \midrule
%         CTracker \cite{chainedtracker} \textbf{\dag} & 66.6 & 57.4 & 32.2 & 24.2 & 22284 & 160491 & 5529 \\
%         CenterTrack \cite{centertrack} & 67.8 & 64.7 & 34.6 & 24.6 & 18489 & 160332 & 3039 \\
%         QDTrack \cite{quasi-dense} \dag & 68.7 & 66.3 & 40.6 & 21.9 & 26598 & 146643 & 3378 \\
%         FairMOT \cite{fairmot} \dag & 69.8 & 69.9 & - & - & - & - & 3996 \\
%         GSDT \cite{gsdt} & 73.2 & 66.5 & 41.7 & 17.5 & 26397 & 120666 & 3891 \\
%         \textbf{SGT (Ours)} \dag & 73.2 & 70.2 & 42.0 & 17.7 & 25332 & 121155 & 4809 \\
%         FairMOT \cite{fairmot} & 73.7 & 72.3 & 43.2 & 17.3 & 27507 & 117477 & 3303 \\
%     \midrule
%     \multicolumn{8}{c}{MOT20 \cite{mot20}} \\
%     \midrule
%         FairMOT \cite{fairmot} & 61.8 & 67.3 & 68.8 & 7.6 & 103440 & 88901 & 5243\\
%         TransTrack \cite{transtrack} & 64.5 & 59.2 & 49.1 & 13.6 & 28566 & 151377 & 3565 \\
%         \textbf{SGT (Ours)} \dag & 64.5 & 62.7 & 62.7 & 10.2 & 67352 & 111201 & 4909 \\
%         CorrTracker \cite{corrtracker} & 65.2 & 69.1 & 66.4 & 8.9 & 79429 & 95855 & 5183 \\
%     \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[t!]
\caption{
Evaluation results of ours and recent online JDT models on the MOT16/17/20 benchmarks (private detection). The values not provided are filled by ``-''. \textbf{\dag}~indicates no extra training dataset.
}
\label{table:sgt_mot_rebuttal}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}l|ccccccc@{}}
    \toprule
    Method & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
    \midrule
    \midrule
    \multicolumn{8}{c}{MOT16} \\
    \midrule
        QDTrack \textbf{\dag} & 69.8 & 67.1 & 41.6 & 19.8 & 9861 & 44050 & 1097 \\
        TraDes  & 70.1 & 64.7 & 37.3 & 20.0 & 8091 & 45210 & 1144 \\
        CSTrack  \textbf{\dag} & 71.3 & 68.6 & - & - & - & - & 1356 \\
        \textbf{SGT (Ours)} \textbf{\dag} & 74.1 & 71.0 & 43.6 & 15.8 & 9784 & 35946 & 1528 \\
        GSDT & 74.5 & 68.1 & 41.2 & 17.3 & 8913 & 36428 & 1229 \\
        FairMOT & 74.9 & 72.8 & 44.7 & 15.9 & - & - & 1074 \\
    \midrule
    \multicolumn{8}{c}{MOT17} \\
    \midrule
        CTracker \textbf{\dag} & 66.6 & 57.4 & 32.2 & 24.2 & 22284 & 160491 & 5529 \\
        CenterTrack & 67.8 & 64.7 & 34.6 & 24.6 & 18489 & 160332 & 3039 \\
        QDTrack \dag & 68.7 & 66.3 & 40.6 & 21.9 & 26598 & 146643 & 3378 \\
        FairMOT \dag & 69.8 & 69.9 & - & - & - & - & 3996 \\
        GSDT & 73.2 & 66.5 & 41.7 & 17.5 & 26397 & 120666 & 3891 \\
        \textbf{SGT (Ours)} \dag & 73.2 & 70.2 & 42.0 & 17.7 & 25332 & 121155 & 4809 \\
        FairMOT & 73.7 & 72.3 & 43.2 & 17.3 & 27507 & 117477 & 3303 \\
    \midrule
    \multicolumn{8}{c}{MOT20} \\
    \midrule
        FairMOT & 61.8 & 67.3 & 68.8 & 7.6 & 103440 & 88901 & 5243\\
        TransTrack & 64.5 & 59.2 & 49.1 & 13.6 & 28566 & 151377 & 3565 \\
        \textbf{SGT (Ours)} \dag & 64.5 & 62.7 & 62.7 & 10.2 & 67352 & 111201 & 4909 \\
        CorrTracker & 65.2 & 69.1 & 66.4 & 8.9 & 79429 & 95855 & 5183 \\
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/threshold_tuning.tex <==


\begin{table}[t!]
    \begin{minipage}[t]{0.23\textwidth}
        \centering
        \caption{Threshold of $\tau_{init}$.}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l|ccccccc@{}}
        \toprule
        $\tau_{init}$ & MOTA$\uparrow$ & IDF1$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
        \midrule
        0.2 & 62.4 & 67.7 & 8687 & 10593 & 1031 \\
        0.3 & 67.7 & 69.7 & 5253 & 11239 & 937 \\
        0.4 & 70.3 & 71.3 & 3388 & 11919 & 758 \\
        0.5 & 71.3 & 73.8 & 2190 & 12742 & 588 \\
        0.6 & 71.0 & 73.8 & 1281 & 14077 & 319 \\
        0.7 & 66.3 & 72.1 & 548 & 17505 & 167 \\
        0.8 & 57.6 & 65.4 & 245 & 22575 & 96 \\
        \bottomrule
        \end{tabular}
        }
        \label{table:init_thresh_tuning}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.23\textwidth}
        \centering
        \caption{Threshold of $\tau_{E}$.}
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l|ccccccc@{}}
        \toprule
        $\tau_E$ & MOTA$\uparrow$ & IDF1$\uparrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
        \midrule
        0.2 & 71.4 & 72.3 & 2783 & 12169 & 514 \\
        0.3 & 71.7 & 74.5 & 2430 & 12347 & 504 \\
        0.4 & 71.3 & 73.8 & 2190 & 12742 & 588 \\
        0.5 & 70.2 & 71.2 & 1882 & 13371 & 827 \\
        0.6 & 69.0 & 69.5 & 1660 & 13944 & 1130 \\
        0.7 & 68.0 & 67.5 & 1549 & 14290 & 1443 \\
        0.8 & 66.7 & 64.0 & 1527 & 14471 & 2024 \\
        \bottomrule
        \end{tabular}
        }
        \label{table:init_thresh_tuning}
    \end{minipage}
    \hfill
\end{table}


% \begin{table}[t!]
%     \centering
%     \caption{
%         Threshold of $\tau_{init}$.
%     }
%     \label{table:init_thresh_tuning}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{@{}l|ccccccc@{}}
%         \toprule
%         Threshold & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%         \midrule
%         0.2 & 62.4 & 67.7 & 53.7 & 11.8 & 8687 & 10593 & 1031 \\
%         0.3 & 67.7 & 69.7 & 51.9 & 13.9 & 5253 & 11239 & 937 \\
%         0.4 & 70.3 & 71.3 & 49.0 & 14.7 & 3388 & 11919 & 758 \\
%         0.5 & 71.3 & 73.8 & 46.6 & 16.2 & 2190 & 12742 & 588 \\
%         0.6 & 71.0 & 73.8 & 44.0 & 20.4 & 1281 & 14077 & 319 \\
%         0.7 & 66.3 & 72.1 & 38.1 & 28.3 & 548 & 17505 & 167 \\
%         0.8 & 57.6 & 65.4 & 29.8 & 38.6 & 245 & 22575 & 96 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}
% \begin{table}[t!]
%     \centering
%     \caption{   
%         Threshold of $\tau_{E}$.
%     }
%     \label{table:edge_thresh_tuning}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{@{}l|ccccccc@{}}
%         \toprule
%         Threshold & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%         \midrule
%         0.2 & 71.4 & 72.3 & 48.4 & 15.6 & 2783 & 12169 & 514 \\
%         0.3 & 71.7 & 74.5 & 47.5 & 15.9 & 2430 & 12347 & 504 \\
%         0.4 & 71.3 & 73.8 & 46.6 & 16.2 & 2190 & 12742 & 588 \\
%         0.5 & 70.2 & 71.2 & 45.4 & 17.4 & 1882 & 13371 & 827 \\
%         0.6 & 69.0 & 69.5 & 42.8 & 17.4 & 1660 & 13944 & 1130 \\
%         0.7 & 68.0 & 67.5 & 42.2 & 18.0 & 1549 & 14290 & 1443 \\
%         0.8 & 66.7 & 64.0 & 41.9 & 18.0 & 1527 & 14471 & 2024 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}

% \begin{table}[t!]
%     \centering
%     \caption{   
%         Threshold of $\tau_{E}$.
%     }
%     \label{table:edge_thresh_tuning}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{@{}l|ccccccc@{}}
%         \toprule
%         Threshold & MOTA$\uparrow$ & IDF1$\uparrow$ & MT$\uparrow$ & ML$\downarrow$ & FP$\downarrow$ & FN$\downarrow$ & IDS$\downarrow$ \\
%         \midrule
%         0.2 & 71.4 & 72.3 & 48.4 & 15.6 & 2783 & 12169 & 514 \\
%         0.3 & 71.7 & 74.5 & 47.5 & 15.9 & 2430 & 12347 & 504 \\
%         0.4 & 71.3 & 73.8 & 46.6 & 16.2 & 2190 & 12742 & 588 \\
%         0.5 & 70.2 & 71.2 & 45.4 & 17.4 & 1882 & 13371 & 827 \\
%         0.6 & 69.0 & 69.5 & 42.8 & 17.4 & 1660 & 13944 & 1130 \\
%         0.7 & 68.0 & 67.5 & 42.2 & 18.0 & 1549 & 14290 & 1443 \\
%         0.8 & 66.7 & 64.0 & 41.9 & 18.0 & 1527 & 14471 & 2024 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}

